Escaping Saddles with Stochastic Gradients

We analyze the variance of stochastic gradients along negative curvature directions in certain non-convex machine learning models and show that stochastic gradients exhibit a strong component along these directions. Furthermore, we show that - contrary to the case of isotropic noise - this variance is proportional to the magnitude of the corresponding eigenvalues and not decreasing in the dimensionality. Based upon this observation we propose a new assumption under which we show that the injection of explicit, isotropic noise usually applied to make gradient descent escape saddle points can successfully be replaced by a simple SGD step. Additionally - and under the same condition - we derive the first convergence rate for plain SGD to a second-order stationary point in a number of iterations that is independent of the problem dimension.

==> sgd-analysis-new.tex <==


\section{\textcolor{red}{Corrections (A FAILED ATTEMPT)}}

So far, we have exploited the variance of stochastic gradients only in the first iteration; hence, we had to periodically increase the step-size to boost the variance along the negative curvature. The question is if we exploit the variance along the negative curvature in all iterations, can we use a constant step-size throughout all iterations? Let's consider SGD with constant step-sizes as
\begin{align} \label{eq:sgd_step_expansion}
\w_{t+1} & = \w_t - \eta \gf(\w_t) + \eta \underbrace{(\gf(\w_t) - \gf_\z(\w_t))}_{\zeta_t}, \quad  \pw = \w_0,
\end{align}
where $\zeta_t$s are zero-mean vectors obtained by the noise of stochastic gradients. We further assume that stochastic gradients are Lipschitz continuous, namely 
\begin{align} \label{eq:lipschitz_stochastic_gradients}
    \| \nabla f_\z(\w_1) - \nabla f_\z(\w_2) \| \leq L \| \w_1- \w_2 \| 
\end{align}
holds for all $\z$s.
\paragraph{Main Idea:} The idea is exploiting the variance of stochastic gradient through all iterations. We consider a tighter lower bound on the expected distance as  
\begin{align} \label{eq:tighter_lowerbound}
    \E \| \w_t - \pw \|^2  \geq \E \| \u_t \|^2 - 2 \eta \| \u_t \| \E \| \bdelta_t \| + \textcolor{blue}{ \eta^2 \E \left[  \| \Omega_t \|^2 \right]}, \quad \Omega_t := \d_t + \bdelta_t + \bzeta_t. 
\end{align}
Note that the last term $\E \| \Omega_t\|^2$ was skipped in the derivation of Eq.~\eqref{eq:tighter_lowerbound}. The noise of all stochastic gradients is included in this term. The goal is to establish a strictly positive lowerbound on this term. 
\paragraph{Why did this approach fail?} Unfortunately, we could noy establish a positive lowerbound on $\E \|\Omega_t \|^2 $. This term can be decomposed as
\begin{align}
     \E \| \Omega_t \|^2 \geq \E \| \bzeta_t \|^2 + 2 \underbrace{\E\left[ \bzeta^\top_t \right]}_{=0} \d_t - 2 \max(\| \bzeta_t \|)  \E \left[  \| \bdelta_t \|  \right] 
\end{align}
Exploiting the negative curvature through all iterations allows us to established a lowerbound on $\E \| \bzeta_t \|^2$. However, we could not established a tight upperbound on the negative term. Undesirably, we ended up with a negative lower-bound, which is useless. In the rest of this section, we present all established upperbounds and lowerbounds that we achieved during this attempt. If one can improve bounds, we might be able to exploit the negative curvature in all iterations. 
\paragraph{Step I.: Negative Curvature Exploitation in Long Run} The question is the stochastic gradients at step $t$, i.e. $\gf_\z(\w_t)$, can signal the negative curvature at the initial parameter $\pw$. Next lemma, establishes a lowerbound on the variance of $\gf_\z(\w_t)$ along the negative curvature $\nabla^2 f(\pw)$. 
\begin{framed}
\begin{lemma}
    Suppose Assumptions \ref{ass:CNC} and \ref{ass:smoothness} hold and stochastic gradients are Lipschitz. Let $\v$ be eigenvector of $\nabla^2 f(\w_0)$ associated with eigenvalue $\lambda_{\min} (\nabla^2 f(\w_0))$.  We further assume that $\E \left[ (\v^\top \nabla f_\z(\w_0))^2  \right] = \sigma^2 >0$. If the function value has not decrease more than $\ft$ in expectation after $k$ iterations, i.e. 
    \begin{align}
       \E \left[ f( \w_{t})  \right] - f(\w_0)   \geq - \ft 
    \end{align}
(we assume that in all iterations  a small step sizes $\eta$ (hence $k < \tr$) is used), then
\begin{align} 
  \E \left[ (\v^\top \nabla f_\z(\w_{t}))^2\right] & \geq \sigma^2 - 2 \sigma L \sqrt{\Delta_t}
\end{align} 
holds where both of the above expectations are taken over the sequence $\{\w_j\}_{1}^{t}$ and $\z$. 
\end{lemma}
\end{framed}
\begin{proof}
\begin{align} 
    \E \left[ (\v^\top \nabla f_\z(\w_{t}))^2 \right] & = \E \left[ (\v^\top (\nabla f_\z(\w_{t}) \mp \nabla f_\z(\w_0))^2\right]   \\
    & \geq \E \left[ (\v^\top \nabla f_\z(\w_0) )^2  \right] - 2  |\E \left[ (\v^\top \nabla f_\z(\w_0))  (\v^\top (\nabla f_\z(\w_{t}) - \nabla f_\z(\w_0))) \right]| \\ 
    & 
    \geq \E \left[ (\v^\top \nabla f_\z(\w_0) )^2  \right] - 2  \left( \E \left[ (\v^\top \nabla f_\z(\w_0))^2 \right] 
    \E \left[ (\v^\top (\nabla f_\z(\w_{t}) - \nabla f_\z(\w_0)))^2 \right] \right)^{1/2} \label{eq:upperbound_on_shifted_variance}
\end{align}
where we used Cauchy-Schwarz inequality in the last step. 
Lipschitzness of the stochastic gradient yields the following upperbound
\begin{align}
    \E \left[ \left(\v^\top   (\nabla f_\z(\w_t) - \nabla f_\z(\w_0) \right)^2 \right] & \leq \E \left[  \| \v \|^2 \|\nabla f_\z(\w_t) - \nabla f_\z(\w_0) \|^2  \right] 
    \\ 
    & \leq L \E \| \w_t - \w_0 \|^2 
\end{align}
Using the above results and using the compact notation $\E \left[ (\v^\top \nabla f_\z(\w_0))^2  \right] = \sigma^2 \geq \gamma $, we further simplify the upperbound of Eq.~\eqref{eq:upperbound_on_shifted_variance} as 
\begin{align} 
\E \left[ (\v^\top \nabla f_\z(\w_{t}))^2\right] & \geq \sigma^2 - 2 \sigma L \left( \E \left[ \| \w_{t} - \w_0 \|^2 \right] \right)^{1/2}
\end{align} 
which concludes the proof. 
\end{proof}
Let's consider the compact notation 
\begin{align}
    \Delta_t : = \max_{k<t} \E \| \w_k - \pw \|^2 
\end{align}
Next corollary shows: for a small enough $\Delta_t$, the stochastic gradient $\gf_\z(\w_t)$ obtains the considerable variance along the negative curvature of $\nabla^2 f(\pw)$.
\begin{corollary} \label{cor:long_curvature_exploitation}
Under the assumption of the last lemma, if $\E \left[ (\v^\top \nabla f_\z(\w_0))^2  \right] = \sigma \geq \gamma$ such that 
\begin{align}
   \Delta_t \leq \gamma/8  
\end{align}
Then 
\begin{align} 
  \E \left[ (\v^\top \nabla f_\z(\w_{t}))^2\right] & \geq \frac{1}{2}\gamma
\end{align} 
holds where both of the above expectations are taken over the sequence $\{\w_j\}_{1}^{t}$ and $\z$. 
\end{corollary} 
\begin{proof}
Using the result of the last lemma, we have 
\begin{align}
    \E \left[ (\v^\top \nabla f_\z(\w_{t}))^2\right] & \geq \sigma^2 - 2 \sigma L \left( \E \left[ \| \w_{t} - \w_0 \|^2 \right] \right)^{1/2} \\ 
    & \geq \sigma^2 - \sigma \sqrt{\gamma}/2 \\ 
    & \geq \sigma^2 - \sigma^2/2  \\ 
    & \geq \sigma^2/2 \geq \gamma/2 
\end{align}
\end{proof}
The required upperbound on $\Delta_t$ in the last corollary can be achieved by choosing sufficiently small step size according to Lemma~\ref{lemma:expected_distance_bound} (So far so good).
\paragraph{Step II. Exploiting the variance in a long run}

Using the result of corollary~\ref{cor:long_curvature_exploitation}, next lemma establishes a lowerbound on $\E \left[\| \bzeta_t \|^2\right]$ of Eq.~\ref{eq:tighter_lowerbound}.  
\begin{framed}
\begin{lemma} \label{lemma:explosive_stochastic_gradients}
Under the assumption of the last lemma, if $\E \left[ (\v^\top \nabla f_\z(\w_0))^2  \right] = \sigma \geq \gamma$ such that 
\begin{align} \label{eq:distance_assumption}
    \Delta_t \leq \frac{\gamma}{8 \max\{1 , L\}} , \quad \forall i < t   
\end{align}
Then 
\begin{align}
    \E \left[ \| \bzeta_t \|^2 \right] \geq \sum_{i=1}^{2t} \kappa^{i} \left( \gamma/8  -  \| \gf(\pw) \|^2 \right) 
\end{align}
as long as $\gamma/8> \| \gf(\pw)\|^2$. 
\end{lemma}
\end{framed}
\begin{proof}
  \begin{align}
      \E \left[ \| \bzeta_t \|^2 \right] = \E \left[ \| \sum_{i=1}^t (\Im - \eta \H)^{t-i} \zeta_i  \right]  = \sum_{i,j} \E \left[\langle (\Im - \eta \H)^{t-i} \zeta_i, (\Im - \eta \H)^{t-j} \zeta_j \rangle \right]
  \end{align}
  The result of lemma~\ref{lemma:zero_covariance_law} that the above cross-product is zero for $i \neq j$, hence 
  \begin{align}
      \E \left[ \| \bzeta_t \|^2 \right] & = \sum_{i=1}^t \E \left[ \| (\Im - \eta \H)^{t-i} \zeta_i \|^2 \right] \\ 
      & = \sum_{i=1}^t \E \left[ \| \left( \Im - \eta \H\right)^{t-i} \left( \gf_{r_i}(\w_i) - \gf (\w_i) \right) \|^2 \right] \\ 
      & = \sum_{i=1}^t \left( \E \left[ \|\left( \Im - \eta \H\right)^{t-i} \gf_{r_i}(\w_i)\|^2  \right] - \E \left[ \|\left( \Im - \eta \H\right)^{t-i} \gf(\w_i) \|  \right] \right) \\ 
      & \geq \sum_{i=1}^t \kappa^{2i} ( \gamma/2 - \E \left[ \| \nabla f(\w_i) \|^2  \right]) , \quad \text{lemma~\ref{lemma:lower_bound_u_2} and corollary~\ref{cor:long_curvature_exploitation}} \label{eq:lowerbound_on_norm_of_bzeta_1}
  \end{align}
  Using the smoothenss assumption, we can further bound expected gradient as 
  \begin{align}
       \E \| \gf (\w_i) \|^2 & = \E \| \gf(\w_i) \mp \gf(\pw) \|^2 \\ 
       & \leq  2 L \E \| \w_i - \w \|^2 + 2 \| \gf(\pw) \|^2  \\ 
       & \leq \gamma/4 + 2 \| \gf(\pw) \|^2 
  \end{align}
 Plugining the above result into Eq.~\eqref{eq:lowerbound_on_norm_of_bzeta_1} yields 
 \begin{align} \label{eq:lowerbound_on_norm_of_bzeta_2}
     \E \left[ \| \bzeta_t \|^2 \right] \geq \left( \gamma/4  - 2 \| \gf(\pw) \|^2 \right) \sum_{i=1}^t \kappa^{2i}  
 \end{align}
 Let $a = \sum_{i=1}^t \kappa^{2i}$, then $a/\kappa = \sum_{i=1}^t \kappa^{2i-1}$, hence 
 \begin{align}
     \sum_{i=1}^{2t} \kappa^i = a + a/\kappa = (1+1/\kappa) a 
 \end{align}
 which concludes that 
 \begin{align}
     \sum_{i=1}^t \kappa^{2i} = a = \sum_{i=1}^{2t} \kappa^i/(1+1/\kappa) \geq \sum_{i=1}^{2t} \kappa^{i}/2 
 \end{align}
 Replacing the above result into the lower-bound of Eq.~\eqref{eq:lowerbound_on_norm_of_bzeta_2} completes the proof.  
\end{proof}
\paragraph{Step III. upperbounds}
To reach a positive lowerbound, we need to establish an upperbound on the negative term of Eq.~\eqref{eq:tighter_lowerbound}. 
\begin{lemma} 
[Upper bound on the noise of stochastic gradients] \label{lemma:upperbound_on_noise_of_stochastic_gradients}
Under assumptions of last lemma, $\bzeta_t$ is bounded as 
\begin{align}
    \| \bzeta_t \| \leq  2 \ell \kappa^{t}/(\eta \lambda)
\end{align}
\end{lemma} 
\begin{proof}
\begin{equation}
  \begin{aligned}
      \| \bzeta_t \| & = \| \sum_{i=1}^t \left( \Im - \eta \H \right)^{t-i} \zeta_t \| \\ 
      & \leq \sum_{i=1}^t \| \left( \Im - \eta \H \right)^{t-i} \zeta_t \| \\ 
      & \leq \sum_{i=1} \kappa^{t-i} 2 \ell \\ 
      & \leq \ell \kappa^{t} \sum_{i=1}^t \kappa^{-i} \leq \ell \kappa^{t} \sum_{i=1}^\infty \kappa^{-i}\leq 2 \ell \kappa^{t}/(\eta \lambda)  
  \end{aligned}
 \end{equation}
\end{proof}
\begin{lemma} \label{lemma:new_bound_on_delta_sgd}
Term $\bdelta_t$, presented in Table~\ref{tab:sgd_expansion_vectors} is bounded as 
\begin{align}
 \E \| \bdelta_t \| \leq (\Delta_t \rho/2) \sum_{k=1}^t \kappa^{t-k} 
\end{align}
\end{lemma}
\begin{proof}
  \begin{align}
     \E \| \bdelta_t \| & = \E \| \sum_{k=1}^t \left( \Im - \eta \H  \right)^{t-k} \left( \gf_k - \gg_k \right) \|  \\ 
& \leq \sum_{k=1}^t (1+\eta  \lambda )^{t-k} \E \| \gf_k - \gg_k \| \\ 
& \leq (\rho/2) \sum_{k=1}^t \kappa^{t-k}  \E \| \w_k - \pw \|^2 \quad \quad \text{[Lipshitz Hessian Assumption].}
  \end{align}
\end{proof}
\paragraph{A Possibly Negative Lowerbound} Let $\Delta_t = \max_{k<t} \E \| \w_k - \pw \|^2$. Here, we use the established bounds in last 3 lemmas to lower bound $\Omega_t$: 
\begin{align}
    \E \| \Omega_t \|^2 & \geq \E \| \bzeta_t \|^2  - 2 \| \bzeta_t \| \E \left[  \| \bdelta_t \|  \right] \\ 
    & \geq \sum_{i=1}^{2t} \kappa^{i} \left( \gamma/8  - \| \gf(\pw) \|^2 \right) -2\| \bzeta_t \| \E \left[  \| \bdelta_t \|  \right]  , \quad \text{[Lemma~\ref{lemma:explosive_stochastic_gradients}]} \\ 
    &  \geq \sum_{i=1}^{2t} \kappa^{i} \left( \gamma/8  - \| \gf(\pw) \|^2 \right) -  2 \ell \kappa^{t}/(\eta \lambda) \E \| \bdelta_t \| \quad \text{[Lemma~\ref{lemma:upperbound_on_noise_of_stochastic_gradients}]} \\ 
    & \geq  \sum_{i=1}^{2t} \kappa^{i} \left( \gamma/8  - \| \gf(\pw) \|^2 \right) - \ell (\Delta_t \rho/\eta \lambda ) \sum_{k=1}^t \kappa^{2t-k} \\ 
    & \geq  \left( \gamma/8 - \| \gf(\pw) \|^2 - \ell (\Delta_t \rho/\eta\lambda) \right) \sum_{i=1}^{2t} \kappa^{i}
\end{align}
To have a positive lowerbound, we need $\Delta_t$ to be bounded as 
\begin{align} 
    \Delta_t \leq  \lambda \eta  \gamma/(32 \ell \rho) 
\end{align}
Since the number of $\tr$ is always $\bigo((\eta \lambda)^{-1})$ (see Eq.~\eqref{eq:sgd_tr_bound}), we can not guarantee the positiveness of the above lowerbound by tuning the step-size $\eta$ using the upperbound of lemma~\ref{lemma:expected_distance_bound_sgd}. We have also tried to improve the upperbound of Lemma \ref{lemma:expected_distance_bound_sgd}, but it did not work out.





